A Systematic Survey of Prompt Engineering in Large Language Models: Techniques and Applications

Prompt engineering has emerged as an indispensable technique for extending the capabilities of large language models (LLMs) and vision-language models (VLMs). This approach leverages task-specific instructions, known as prompts, to enhance model efficacy without modifying the core model parameters. Rather than updating the model parameters, prompts allow seamless integration of pre-trained models into downstream tasks by eliciting desired model behaviors solely based on the given prompt. Prompts can be natural language instructions that provide context to guide the model or learned vector representations that activate relevant knowledge. This burgeoning field has enabled success across various applications, from question-answering to commonsense reasoning. However, there remains a lack of systematic organization and understanding of the diverse prompt engineering methods and techniques. This survey paper addresses the gap by providing a structured overview of recent advancements in prompt engineering, categorized by application area. For each prompting approach, we provide a summary detailing the prompting methodology, its applications, the models involved, and the datasets utilized. We also delve into the strengths and limitations of each approach and include a taxonomy diagram and table summarizing datasets, models, and critical points of each prompting technique. This systematic analysis enables a better understanding of this rapidly developing field and facilitates future research by illuminating open challenges and opportunities for prompt engineering.

==> table.tex <==
\begin{center}
\begin{table*}[h!]
\centering
\footnotesize
% \scriptsize
\scalebox{0.85}{
\begin{tabular}{|l|c|c|c|c|}
\hline
Category & \begin{tabular}[c]{@{}c@{}}Prompting Technique \end{tabular} & \begin{tabular}[c]{@{}c@{}}Evaluated \\ LLM(s) \end{tabular} & Dataset(s) & \begin{tabular}[c]{@{}c@{}}Task(s) \end{tabular} \\
\hline
\begin{tabular}[c]{@{}c@{}}New Tasks Without \\Training Data \end{tabular}  & Zero-shot Prompting  & - & - & - \\ 
\cline{2-5}

& Few-shot Prompting  & - & - & - \\ 
\hline

 & Chain-of-Thought~\cite{wei2022chain} & \begin{tabular}[c]{@{}c@{}}PaLM 540B, \\ code-davinci-002, \\text-davinci-002,\\LaMDA 137B  \end{tabular}  
 & \begin{tabular}[c]{@{}c@{}}Arithmetic Reasoning[\\ GSM8K, \\SVAMP,\\ASDiv, \\ AQuA, \\MAWPS] \\ Commonsense \\ Reasoning [\\ CSQA,\\StrategyQA,\\ Date, \\Sports, \\SayCan] \\ Symbolic\\ Reasoning [ \\Letter, \\ Coin] \end{tabular}  & \\ 
 
 \cline{2-5}

%  arithmetic(GSM8K ,SVAMP ,ASDiv ,AQuA ,MAWPS)
% commonsense reasoning (CSQA ,StrategyQA, Date, Sports, SayCan)
% symbolic reasoning(Letter, Coin) 
 
 & \begin{tabular}[c]{@{}c@{}}Automatic \\ Chain-of-Thought~\cite{zhang2022automatic} \end{tabular} & \begin{tabular}[c]{@{}c@{}}PaLM 540B, \\GPT-3,\\LaMDA 137B \end{tabular} & \begin{tabular}[c]{@{}c@{}}Arithmetic Reasoning[\\ GSM8K, \\SVAMP,\\ASDiv, \\ AQuA, \\MAWPS] \\ Commonsense \\ Reasoning [\\ CSQA,\\StrategyQA,\\ Date, \\Sports, \\SayCan] \\ Symbolic\\ Reasoning [ \\Letter, \\ Coin] \end{tabular}  & \\ 
 \cline{2-5}

Reasoning and Logic   & Self-Consistency~\cite{wang2022self} &
\begin{tabular}[c]{@{}c@{}} UL2-20B,\\PaLM 540B,\\code-davinci-002,\\
text-davinci-002,\\ LaMDA 137B \end{tabular} & \begin{tabular}[c]{@{}c@{}}Arithmetic Reasoning[\\ GSM8K, \\SVAMP,\\ASDiv, \\ AQuA, \\MAWPS] \\ Commonsense \\ Reasoning [\\ CSQA,\\StrategyQA,\\ Date, \\Sports, \\SayCan] \\ Symbolic\\ Reasoning [ \\Letter, \\ Coin] \end{tabular}  &  \\ 
  \cline{2-5}
  
& Tree-of-Thoughts~\cite{yao2023tree} & GPT-4 & \begin{tabular}[c]{@{}c@{}} Game of 24,\\ Creative Writing,\\ Mini Crosswords \end{tabular} & \\
\cline{2-5}

& Graph-of-Thought~\cite{yao2023beyond}  & \begin{tabular}[c]{@{}c@{}} GPT-3, \\GPT-3.5,\\GPT-4,\\code-davinci-002,\\T5(base \& large) \end{tabular}& \begin{tabular}[c]{@{}c@{}} GSM8K,\\ ScienceQA\end{tabular} &  \\ 
\cline{2-5}

& System 2 Attention~\cite{weston2023system}  & \begin{tabular}[c]{@{}c@{}} GPT-4, \\ LLaMA-2-70B\end{tabular}& \begin{tabular}[c]{@{}c@{}} QA,\\ math word problems\\longform \end{tabular} &  \\ 

  \hline
 & Chain-of-Verification~\cite{dhuliawala2023chain} & \begin{tabular}[c]{@{}c@{}} Llama 2 70B Chat,\\ Llama 65B \end{tabular} & \begin{tabular}[c]{@{}c@{}} Wikidata,\\ QUEST,\\ MultiSpanQA\end{tabular}&  \\  
 \cline{2-5}
 
 &  ReAct Prompting~\cite{yao2022react} & \begin{tabular}[c]{@{}c@{}}PaLM-540B,\\ GPT-3\end{tabular} & \begin{tabular}[c]{@{}c@{}} HotpotQA,\\ Fever,\\ALFWorld,\\ WebShop\end{tabular}&  \\  
 \cline{2-5}
 
Reduce Hallucination & \begin{tabular}[c]{@{}c@{}}Retrieval Augmented \\ Generation~\cite{lewis2020retrieval} \end{tabular} & \begin{tabular}[c]{@{}c@{}}T5-11B, \\RAG-Token,\\ RAG-Seq.,\\REALM,\\DPR \end{tabular} &  \begin{tabular}[c]{@{}c@{}} Natural Questions,\\ TriviaQA,\\WebQuestions \\and CuratedTrec,\\MSMARCO NLG\\ task v2.1,\\SearchQA, \\Fever \end{tabular} & \\  
\cline{2-5}
\end{tabular}
}
\caption{A comparative summary of the literature and the proposed model}
\label{tab:comparison}
\end{table*}
\end{center}


\begin{center}
\begin{table*}[h!]
\centering
\footnotesize
% \scriptsize
\scalebox{0.85}{
\begin{tabular}{|l|c|c|c|c|}
\hline
Category & \begin{tabular}[c]{@{}c@{}}Prompting Technique \end{tabular} & \begin{tabular}[c]{@{}c@{}}Evaluated \\ LLM(s) \end{tabular} & Dataset(s) & \begin{tabular}[c]{@{}c@{}}Task(s) \end{tabular} \\
\hline

 & Chain-of-Note~\cite{yu2023chainofnote} & \begin{tabular}[c]{@{}c@{}} LLaMa-2,\\ DPR \end{tabular} & \begin{tabular}[c]{@{}c@{}} NQ,\\ TriviaQA, \\WebQ \end{tabular} &  \\ \cline{2-5}
 
 & Chain-of-Knowledge~\cite{li2023chainofknowledge} & gpt-3.5-turbo-0613 & \begin{tabular}[c]{@{}c@{}} Factual [\\ FEVER,\\ HotpotQA,\\FeTaQA]\\
Medical [\\MedMCQA] \\ Physics [ \\MMLU Physics]\\Biology [\\MMLU Biology]\end{tabular} &  \\  \hline 

 User Interaction & Active-Prompt~\cite{diao2023active} & \begin{tabular}[c]{@{}c@{}} CodeX code-davinci-002, \\text-davinci-002, \\ text-davinci-003 \end{tabular} & \begin{tabular}[c]{@{}c@{}}Arithmetic [\\ GSM8K, \\SVAMP,\\ASDiv, \\ AQuA, \\MAWPS] \\ Commonsense \\ Reasoning [\\ CSQA,\\StrategyQA,\\ Date, \\Sports, \\SayCan] \\ Symbolic\\ Reasoning [ \\Letter, \\ Coin] \end{tabular}  &  \\ 
 \hline
 % & Instruction Prompting and Tuning &  & \xmark &  \\ \hline

 % & & \xmark & \cmark& FedAWA \\ \hline 

\begin{tabular}[c]{@{}c@{}} Fine-Tuning and \\ Optimization \end{tabular}   & \begin{tabular}[c]{@{}c@{}}Automatic Prompt \\ Engineer~\cite{zhang2022automatic} \end{tabular}   & \begin{tabular}[c]{@{}c@{}} Ada, \\ babbage,\\ curie,\\ davinci,\\ text-ada-001,\\ text-babbage-001,\\ text-curie-001,\\ text-davanci-002 \end{tabular} & \begin{tabular}[c]{@{}c@{}} 24 Instruction Induction,\\
BIG-Bench Instruction Induction \\(emotional understanding,\\ context-free question answering,\\ reading comprehension,\\ summarization, \\algorithms,\\ and various reasoning tasks) \\
TruthfulQA \end{tabular}&  \\ \hline

% & Automatic Prompt Engineer (APE) & \xmark & \cmark& FAVOR \\ \hline

\begin{tabular}[c]{@{}c@{}} Knowledge-Based\\Reasoning and
Generation \end{tabular}  & \begin{tabular}[c]{@{}c@{}} Automatic Reasoning\\and Tool-use~\cite{paranjape2023art} \end{tabular}  & \begin{tabular}[c]{@{}c@{}} GPT-3 (175B),\\Toolformer,\\InstructGPT \\(text-davinci-002)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}SQUAD, \\TriviaQA,\\ SVAMP,\\ MAWPS,\\ MMLU \end{tabular} &  \\ \hline

 % & Retrieval Augmented Generation (RAG) & \xmark & \cmark& FAVOR \\ \hline

\begin{tabular}[c]{@{}c@{}} Improving Consistency\\and Coherence \end{tabular} & \begin{tabular}[c]{@{}c@{}} Contrastive\\Chain-of-Thought~\cite{chia2023contrastive} \end{tabular}   & GPT-3.5-Turbo (0301) & \begin{tabular}[c]{@{}c@{}} arithmetic [ \\GSM8K,\\SVAMP,\\ASDiv,\\AQuA,\\GSM-Hard] \\Factual QA [\\Bamboogle\\ StrategyQA] \end{tabular}&  \\ \hline

\begin{tabular}[c]{@{}c@{}} Managing Emotions\\and Tone \end{tabular} 
   & Emotion Prompting~\cite{li2023large} & \begin{tabular}[c]{@{}c@{}} T5,\\ Vicuna,\\ BLOOM,\\ Llama 2,\\ gpt-3.5-turbo,\\ GPT-4 \end{tabular}& \begin{tabular}[c]{@{}c@{}} 24 instruction \\ induction tasks, \\BIG-Bench \\Instruction \\Induction (BBII) \end{tabular}&  \\ \hline

 & \begin{tabular}[c]{@{}c@{}}Structured  \\ Chain-of-Thought~\cite{zhang2022automatic}\end{tabular} & \begin{tabular}[c]{@{}c@{}} ChatGPT, \\Codex \end{tabular}& \begin{tabular}[c]{@{}c@{}} HumanEval,\\ MBPP,\\MBCPP \end{tabular} & \\
 \cline{2-5}
  %& Program of Thoughts & \cmark& FAVOR \\ \cline{2-5}

 & Program of Thoughts~\cite{chen2022program} & \begin{tabular}[c]{@{}c@{}}code-davinci-002,\\ text-davinci-002,\\
 gpt-3.5-turbo,\\PaLM,\\codegen-16B\end{tabular} &\begin{tabular}[c]{@{}c@{}} GSM8K,\\AQuA,\\SVAMP,\\TabWMP,\\FinQA,\\ConvFin,\\TATQA \end{tabular}&  \\ \cline{2-5}

\begin{tabular}[c]{@{}c@{}}Code Generation and \\ Execution\end{tabular}   & Chain of Code Prompting~\cite{li2023chain} & \begin{tabular}[c]{@{}c@{}}text-ada-001, \\text-baggage-001, \\text-curie-001,\\text-davinci-003,\\gpt-3.5-turbo,\\gpt-4 \end{tabular} & \begin{tabular}[c]{@{}c@{}} BIG-Bench\\ Hard (BBH) - 23 tasks[ \\semantic reasoning, \\numerical reasoning, \\combination of \\semantic and \\numerical reasoning] \end{tabular} &  \\ \cline{2-5}

 & Scratchpad Prompting~\cite{nye2021show} & GPT  & \begin{tabular}[c]{@{}c@{}} MBPP,\\MBPP-aug \end{tabular}&  \\ \hline

\begin{tabular}[c]{@{}c@{}}Optimization \\and Efficiency\end{tabular}  & Optimization by Prompting~\cite{yang2023large} & \begin{tabular}[c]{@{}c@{}} text-bison,\\ PaLM 2-L,\\PaLM 2-L-IT,\\ gpt-3.5-turbo,\\gpt-4 \end{tabular}& \begin{tabular}[c]{@{}c@{}}GSM8,\\Multi-Arith,\\AQuA \end{tabular}&  \\ \hline

Understanding User Intent & Rephrase and Respond~\cite{deng2023rephrase} & \begin{tabular}[c]{@{}c@{}}GPT-3.5-turbo-0613,\\ Vicuna-13b-v1.5, \\GPT-4-0613 \end{tabular}  & \begin{tabular}[c]{@{}c@{}}Knowledge Classification [\\Even day,\\Even month,\\Even year,\\Compare age]\\Commonsense Reasoning [\\CSQA,\\Dates]\\Symbolic Reasoning [ \\Last letter (2), \\Last letter (4),\\ Coin flip,\\ Sports] \end{tabular} &  \\ \hline

\begin{tabular}[c]{@{}c@{}} Metacognition and\\Reflection \end{tabular} & \begin{tabular}[c]{@{}c@{}}Take a Step \\Back ~\cite{zheng2023take} \end{tabular}   &\begin{tabular}[c]{@{}c@{}} PALM2-L,\\ GPT-4 \end{tabular}&\begin{tabular}[c]{@{}c@{}} TimeQA,\\ StrategyQA,\\ MMLU high-school\\ Physics,\\MuSiQue \end{tabular}&  \\ \hline

\end{tabular}
}
\caption{A comparative summary of the literature and the proposed model}
\label{tab:comparison}
\end{table*}
\end{center}




==> table2.tex <==
\begin{table*}
\begin{center}
 \caption{The performance evaluation of the proposed model using BERTScore.}
\label{cla_result2}
\scalebox{1}{
\begin{tabular}{c|c|c|c|c|c|c}
% \hline
% &&&&{ROUGE Score} \\
\hline
{Evaluation Metrics}
&\multicolumn{2}{c|}{BLIP} &
\multicolumn{2}{c|}{GIT} &
\multicolumn{2}{c}{InstructBLIP}  \\
\cline{2-7}
    &Base &Fine-Tune & Base &Fine-Tune & Base &Fine-Tune \\
\hline
Precision (\%) & 81.92 & 84.04 & 82.64 & 86.64 & 83.27 & \textbf{89.64}\\
Recall (\%) & 78.32 & 81.95 & 79.09 & 83.09 & 78.09 & \textbf{89.12} \\
F1-score (\%) & 80.05 & 82.98 & 81.21 & 85.21 & 80.57 & \textbf{89.31} \\
\hline
\end{tabular}
}
\end{center}
\end{table*}
